Pack and Detect: Fast Object Detection in Videos Using Region-of-Interest Packing

Object detection in videos is an important task in computer vision for various applications such as object tracking, video summarization and video search. Although great progress has been made in improving the accuracy of object detection in recent years due to the rise of deep neural networks, the state-of-the-art algorithms are highly computationally intensive. In order to address this challenge, we make two important observations in the context of videos: (i) Objects often occupy only a small fraction of the area in each video frame, and (ii) There is a high likelihood of strong temporal correlation between consecutive frames. Based on these observations, we propose Pack and Detect (PaD), an approach to reduce the computational requirements of object detection in videos. In PaD, only selected video frames called anchor frames are processed at full size. In the frames that lie between anchor frames (inter-anchor frames), regions of interest (ROIs) are identified based on the detections in the previous frame. We propose an algorithm to pack the ROIs of each inter-anchor frame together into a reduced-size frame. The computational requirements of the detector are reduced due to the lower size of the input. In order to maintain the accuracy of object detection, the proposed algorithm expands the ROIs greedily to provide additional background around each object to the detector. PaD can use any underlying neural network architecture to process the full-size and reduced-size frames. Experiments using the ImageNet video object detection dataset indicate that PaD can potentially reduce the number of FLOPS required for a frame by $4\times$. This leads to an overall increase in throughput of $1.25\times$ on a 2.1 GHz Intel Xeon server with a NVIDIA Titan X GPU at the cost of $1.1\%$ drop in accuracy.

==> Athindran_body.tex <==
\section{Introduction}
The task of object detection in videos \cite{KangTCNN16,zhu2017deep,Kang_2016_CVPR,Kang2017object,zhu2017flow,Zhu_2018_CVPR,TSSD,pan2018recurrent,mobilevideo,fastYOLO} has been gaining attention in recent years. It can serve as an important preprocessing task primarily for object tracking and for several other video processing tasks such as video summarization and video search. Further, object detection and tracking can aid  various important applications such as traffic monitoring, pedestrian tracking, animal monitoring and environment survey using drones. Many of these applications require video frames to be processed in real-time in resource-constrained environments. It is thus imperative to design systems that can detect objects in videos in a fast, compute-light and accurate manner.
\par
 Still-image object detection has been studied extensively in the past. The accuracy and speed of still-image object detection have improved by leaps and bounds in recent years due to innovations in the usage of deep convolutional neural networks (CNN) for object detection. The state-of-the-art CNN based still-image object detectors currently are faster RCNN \cite{NIPS2015_FRCNN}, SSD \cite{liu2016ssd}, YOLO \cite{CVPR_YOLO,yolo9000,yolov3} and RFCN\cite{dai2016r}. SSD and YOLO are almost $7-10 \times$ faster than faster-RCNN and RFCN and give comparable accuracy (mAP score) on standard still-image object detection datasets. 
\par
These still-image object detectors can be extended for object detection in videos by using them on a per-frame basis. However, this is inefficient as there is a strong temporal correlation between frames in a video. This temporal redundancy can be leveraged either to improve the accuracy or speed of object detection. In the recent past, there have been several attempts to improve the accuracy of object detection in videos by either integrating the bounding boxes \cite{KangTCNN16,Kang_2016_CVPR,han2016seq,penglinking} or features \cite{Kang2017object,zhu2017flow,Zhu_2018_CVPR,hetangimpression} across frames. However, there has not been enough attention on leveraging this temporal redundancy to improve speed. Some exceptions to this norm are \cite{zhu2017deep,TSSD,pan2018recurrent,mobilevideo,fastYOLO}. In this work, we propose a method, Pack and Detect (PaD), for fast object detection in videos with negligible loss in accuracy.
\par
Neural networks are in general very computationally intensive. For example, processing a video at $300 \times 300$ resolution using the SSD300 (Single Shot Detector) object detection network with VGG16 as backbone at 30 fps requires 1.87 trillion FLOPS/s. Several attempts \cite{szesurvey} have been made to make them less compute-hungry. Techniques such as pruning weights or connections \cite{HanMD15,Han2015}, pruning filters in full or part in a CNN \cite{thinet,NIPS2016_ssparsity,Guo2017,deepakrandom,haopruning}, reducing the precision of floating point operations \cite{AxNNvenkat,anwarprecision} and designing compute-light architectures \cite{mobilenet,squeezenet} have proven to be successful in the past. While most of these methods are static and are employed at design time, there are some methods such as conditional computation \cite{bengiocondcomp}, dynamic deep neural networks (D2NN) \cite{LiuD17} and dynamic variable effort deep neural networks \cite{GanapathyVRR17} (DyVEDEEP) that dynamically adjust the amount of computation to be employed for an input. However, firstly, all of these methods do not exploit the specific opportunities that can be leveraged in the context of videos. Secondly, all of these methods try to modify the network and do not try to compress the inputs to be fed into the network.
\par
In particular, there are two opportunities we are trying to leverage in the context of videos. Firstly, the objects of interest have been observed to occupy only a small fraction of the area in an image. Secondly, there is a strong temporal correlation between frames in a video. We propose Pack and Detect (PaD) which leverages these two opportunities. The full-sized image is only processed in selected frames called anchor frames. In the frames between the anchor frames (inter-anchor frames), the detections from the previous frame are used to identify regions in the image where an object could potentially be located. These regions are called regions of interest (ROIs). The ROIs are packed in a lower sized image which is fed into the detector.
\par 
We propose a ROI packing algorithm based on a greedy heuristic that is responsible for packing the ROI's in the lower-sized frame while meeting the following criteria:
\begin{enumerate}
\item Each ROI is expanded to provide as much background context as possible to maintain the accuracy of the detector.
\item There is minimal loss of resolution and no change in aspect ratio to maintain the accuracy of the detector.
\item Each object is present in an unique ROI. 
\item The space in the lower-sized frame is used as efficiently and impartially as possible.
\end{enumerate}
\par
Our method, PaD,  which uses the ROI-packing algorithm to compress the input in inter-anchor frames is naturally faster because of the smaller size of the input fed to the object detector. In the inter-anchor frames, the FLOP count can potentially reduce by a factor of $4\times$. Tuning the algorithm parameters can provide a $1.3\times$ increase in throughput with only a $2.5\%$ drop in accuracy compared to a baseline mechanism that uses the object detector on a per-frame basis. We vary different parameters of the algorithm to achieve a tradeoff between speed and accuracy. Further, we present results that provide insight into the inner workings of the algorithm. 
\par
In section \ref{sec:rel_work}, we review some of the related work. In section \ref{sec:motivation}, we analyze the two opportunities we are trying to leverage in the context of videos. In section \ref{sec:Methodology}, we provide a overview of the methods and algorithms used in our work. Section \ref{sec:experiment} outlines the experimental methodology and section \ref{sec:results} reports the results obtained from our experiments. In section \ref{sec:conclusion}, we conclude our work.

\section{Related Work}
\label{sec:rel_work}
\subsection*{Object Detection in Videos}
The temporal redundancy in videos has been exploited before to improve the accuracy and speed of object detection in videos. In \cite{KangTCNN16,Kang_2016_CVPR,han2016seq,penglinking}, the aggregation of information from neighbouring frames is done at the bounding box level to improve accuracy. In \cite{KangTCNN16}, per-frame object detection is combined with multi-context suppression, motion-guided propagation and object tracking to improve detection accuracy. In \cite{han2016seq,penglinking}, non-maximum suppression is done over bags of frames. In \cite{Kang2017object,zhu2017flow,Zhu_2018_CVPR,hetangimpression}, there is integration of the CNN features across neighbouring frames to improve accuracy. In \cite{Kang2017object}, a CNN is combined with a LSTM (Long Short Term Memory) to obtain temporal features for object detection. In \cite{zhu2017flow, Zhu_2018_CVPR,hetangimpression}, the features from neighbouring frames are aggregated together using optical flow information to improve feature quality. All the methods discussed till now are extremely slow and \cite{KangTCNN16,Kang_2016_CVPR,han2016seq,penglinking,Kang2017object} are not online.
\par
On the other hand, \cite{zhu2017deep,TSSD,pan2018recurrent,mobilevideo,fastYOLO} are relatively faster methods aimed at object detection in a video. The methods in \cite{TSSD,mobilevideo,fastYOLO} are faster by virtue of using a faster still-image object detector or an efficient backbone network. In \cite{zhu2017deep}, the feature maps of the CNN are not computed in all the frames. The feature maps from anchor frames are transferred to neighbouring frames by warping them with optical flow information. Since the features are not recomputed in each frame, this setup is much more faster and compute-efficient. In \cite{pan2018recurrent}, neighbouring frames are subtracted to give rise to a sparse input. This sparse input is processed by the CNN with the EIE \cite{Han2016} hardware accelerator to achieve computational savings. The methods proposed in this paper are vastly different than the methods in the literature to speed-up video object detection. Even though the overall speed-up achieved in an average sense in our work might not be as high as the $5\times$ reported in \cite{zhu2017deep}, PaD can be used alongside the methods in \cite{zhu2017deep} using some simple tricks to increase the efficiency further. Any efficient neural network or faster object detector can be used with PaD as in \cite{TSSD,mobilevideo,fastYOLO} to obtain further speed-up. Finally, PaD does not require any specialized hardware accelerator like in \cite{pan2018recurrent} to obtain computational savings.
\subsection*{Efficient Neural Networks}
There have been efforts to reduce the number of computations of neural networks using various techniques. Deep compression \cite{HanMD15} deployed on a custom hardware accelator\cite{Han2016} can result in considerable amount of savings in computation and speedup for standard neural networks. Deep compression works by pruning weights less than a threshold, quantizing the weights using clustering followed by huffman coding. EIE \cite{Han2016} is an hardware accelerator that can leverage the sparsity of the deep compressed DNN to speed up the network. Since, fine-grained sparsity has not been shown to improve the speed without custom hardware accelerators, there have been techniques to induce structured sparsity\cite{NIPS2016_ssparsity} by pruning filters \cite{thinet,NIPS2016_ssparsity,Guo2017,deepakrandom,haopruning} of a CNN in full or part. MobileNet\cite{mobilenet} replaces the standard convolution with a combination of depth-wise and point-wise convolution to reduce computation. SqueezeNet\cite{squeezenet} utilizes CNN design techniques to reduce the number of computations and memory. Another innovation is the concept of Big-Little neural networks \cite{biglittle} that first try to use a smaller network to process the image. If the little network is not capable of successfully achieving its task in the frame, the bigger network is used to process the image. This method has been shown to reduce computation significantly without much loss in accuracy.
\par
Most of the methods for achieving computational efficiency in neural networks are static methods to be employed at design time. However, there are some exceptions. Conditional computation \cite{bengiocondcomp} selectively activates certain parts of the network depending on the input. The policy for deciding which parts of the network to activate is learnt using reinforcement learning. Dynamic deep neural networks (D2NN) \cite{LiuD17} work in a manner similar to conditional computation and turn on/off regions of the network using reinforcement learning. DyVEDEEP \cite{GanapathyVRR17} is an unique effort to reduce the computations in neural networks dynamically by using three strategies - saturation prediction and early termination, significance driven selective sampling and similarity-based feature map approximation. 
\par
All the methods try to compress or tweak the model/network to reduce computations and achieve speedup. In this work, we compress the inputs that we feed into the network. Hence, PaD is orthogonal to most existing techniques and can be used in combination with other methods.
\subsection*{Visual Attention Mechanism}
Inspired by human vision, there have been several attempts \cite{NIPS2010_4089,Ranzato14,Mnih2014,ba2014multiple,kosiorek2017hierarchical,kahou2015ratm} to reduce computation by processing an image as a sequence of glimpses rather than processing the image as a whole. The notion of a foveal glimpse is somewhat similar to the idea of ROI discussed here. However, there are several important differences. A foveal glimpse is a high resolution crop of an important region in the image that is crucial to the task at hand. In our work, we pack all the ROIs together in a single frame and do not process them sequentially like how glimpses are processed. Further, the most important difference is that the location of ROI's is inferred from the detections in the previous frame in a video and the network does not need to learn where to look through an attention mechanism. Also, a foveal glimpse obtains crops by extracting pixels close to the location target at high resolution and pixels far from the location target at low resolution. We do not do any multi-resolution processing in our work. Hence, our work, though somewhat inspired from the notion of foveal glimpse is considerably different. 
\section{Motivation}
\label{sec:motivation}
\subsection{Occupancy of objects in a image}
In this work, an opportunity that we try to leverage is the fact that most of the pixels in a frame are clutter and the objects of interest occupy only a small fraction of an area in the frame. We back this hypothesis using statistics from a popular video dataset. From a analysis of the ImageNet VID validation set containing $555$ videos with $176126$ frames, we see that the objects occupy only $22.7\%$ of the image on the average. Figure \ref{fig:occupancy} is a histogram of the object occupancy ratio statistics in the dataset. From the figure, we can infer that the in a huge majority of the frames, the objects occupy less than $30\%$ of the area in a frame.
\begin{figure}
  \centering
  \includegraphics[scale=0.4]{ratios_hist.png}
  \caption{Histogram of object occupancy ratio}
  \label{fig:occupancy}
\end{figure}

\subsection{Temporal correlation of object locations in a video}
In general, we can expect a lot of temporal correlation between consecutive frames in a video unless there are sudden camera shifts or missing frames. We observe this hypothesis to be true from a statistical analysis of the ImageNet VID validation set. On the average, the IoU of area containing objects between consecutive frames is $94.4\%$. Figure \ref{fig:ROIoverlap} is a histogram of the object occupancy area IoU statistics between consecutive frames in the dataset. In the figure we can clearly see a sharp peak close to $1$. We exploit this opportunity in our work.
\begin{figure}
  \centering
  \includegraphics[scale=0.4]{ious_hist.png}
  \caption{Histogram of IoU of regions containing objects between consecutive frames}
  \label{fig:ROIoverlap}
\end{figure}
\section{Methodology}
\label{sec:Methodology}
\subsection{Architecture}
The overall architecture of the methodology proposed in this work is presented in figure \ref{fig:arch}. Full-sized video frames are processed at regular intervals (inter-anchor distance $d$). In the other frames, the ROIs are identified based on the locations of the detections from the previous frame. Only detections with a minimum confidence threshold $\tau$ are taken into consideration. ROI is a region which is likely to contain an object. An ROI packing algorithm will try to pack the ROIs in a lower sized frame. If the packing is successful, then the lower sized frame is processed instead, giving rise to computational savings. However, if the packing is not successful, then the frame is processed at full size. Hence, there is an overhead of checking whether ROI packing is possible. Once the lower sized ROI-packed frame is processed using the CNN detector, the object detections in the ROI packed frame have to be transformed to the original frame dimensions. This can easily be done by keeping track of the ROI boundaries in the original frame.
\begin{figure*}
\centering
\begin{tikzpicture}[auto, node distance=3cm and 3 cm,>=latex]
\tikzset{
  base/.style={draw, on grid,align=center, minimum height=8ex},
  proc/.style={base, rectangle, text width=6em},
  test/.style={base, diamond, text width=4em},
  coord/.style={coordinate, on grid},
}
\node[test,xshift=40mm](p0){\small Is frame anchor frame?};
\node[proc,below of = p0](p1){\small Process frame at full size};
\node[proc,right of = p0](p2){\small Infer the ROI's in the frame based on the detections from the previous frame};
\node[proc,right of = p2](p3){\small Run the ROI packing algorithm to pack the ROI's in a lower sized frame};
\node[test, right of = p3](p4){\small Is ROI packing successful?};
\node[proc, below of = p4](p5){\small Process frame at lower size};
\path (p0.south) to node [near start, xshift=0.2em] {$Yes$} (p1);
\draw [*->] (p0.south) -- (p1);
\path (p0.east) to node [near start, xshift=0.2em] {$No$} (p2);
\draw [*->] (p0.east) -- (p2);
\path (p2.east) to node [near start, xshift=0.2em] {} (p3);
\draw [->] (p2.east) -- (p3);
\path (p3.east) to node [near start, xshift=0.2em] {} (p4);
\draw [->] (p3.east) -- (p4);
\path (p4.south) to node [near start, xshift=0.2em] {$Yes$} (p5);
\draw [*->] (p4.south) -- (p5);
\node [coord, above of = p4, yshift=-1em]  (c1)  {};
\node [coord, left of = p1, node distance = 6em] (c2){};
\path (p4.north) to node [xshift=2em] {$No$} (c1);
  \draw [*-] (p4.north) -- (c1) -| (c2);
\path (c2.east) to node [xshift=1em]{}(p1);
  \draw [->] (c2.east) -- (p1);   
\end{tikzpicture}
\caption{Overall Architecture of PaD} \label{fig:arch}
\end{figure*}

\subsection{ROI packing algorithm}
In figure \ref{fig:flow1}, we illustrate the overall flow of our ROI packing algorithm based on a greedy heuristic. This algorithm is key to ensure that there is no significant drop in accuracy due to ROI packing. As a first step in the algorithm, we find all the connected components of all nodes in a graph where nodes represent ROIs and two nodes are connected if their respective ROI's intersect. We then find the enclosing bounding box over the union of ROI's in each connected component. We iterate the connected components algorithm until we ensure that none of the final bounding boxes overlap. This constraint is important because if two bounding boxes overlap, then parts of the same object could be present two or more times in the ROI packed frame.
\par
Once the number and size of the bounding boxes are decided, the layout of the bounding boxes is determined by a heuristic procedure. The flowchart in figure \ref{fig:tiling} illustrates the algorithm used for determining the layout. Simpler variants of this procedure could also be adopted. Once the layout is decided, a check is done to see whether the bounding boxes can fit in the layout. If it is not possible to fit the bounding boxes in the layout, the ROI packing procedure stops here and the image is processed at full size.
\par 
If the bounding boxes can be fit in the layout, the following procedure is carried out. Using experiments, we noted that CNN object detectors are often overfit to the background context of the object to be detected. The performance of the CNN object detector is poor if there is no background context. Hence, we extend each bounding box within the space available for each bounding box in the layout to provide as much context as possible to the CNN detector. The algorithm for extending the bounding boxes works as follows. First, we make a decision using some heuristic rules as to whether to extend the boxes horizontally or vertically first. For the sake of discussion, let us assume that the choice is to extend horizontally all the bounding boxes first. We find all the bounding boxes, which could potentially intersect when extended horizontally. We extend all bounding boxes horizontally until the layout size is reached or the bounding boxes start intersecting with each other. Then we repeat the same procedure in the other dimension. Once the final bounding boxes are decided, the corresponding regions in the image are extracted and the lower sized frame is filled according to the decided layout.
\par
There are a lot of heuristic rules in the ROI packing algorithm. All of these rules have been decided after thorough analysis of the setup using experiments. In section \ref{sec:results}, we show some results illustrating that this sophisticated ROI packing algorithm is superior to a naive ROI packing algorithm. Further, there are two parameters we can tune to achieve a speed-accuracy tradeoff. Firstly, an obvious parameter that can be tuned is the inter-anchor distance $d$. Also, most of the CNN object detectors have some amount of robustness inbuilt to tackle scale variations. Hence, we could fit the ROI's extracted from a $s_{1} \times s_{1}$ sized frame into a $s_{2} \times s_{2}$ frame and downscale the ROI packed frame to $s_{3} \times s_{3}$ to get higher speed-ups. There will be some loss of accuracy due to the downscaling. We explore these trade-offs in section \ref{sec:results}.
\begin{figure*}
\centering
\begin{tikzpicture}[%
    >=triangle 60,              % Nice arrows; your taste may be different
    start chain=going below,    % General flow is top-to-bottom
    node distance=6mm and 60mm, % Global setup of box spacing
    every join/.style={norm},   % Default linetype for connecting boxes
    ]
\tikzset{
  base/.style={draw, on chain, on grid, align=center, minimum height=4ex},
  proc/.style={base, rectangle, text width=30em},
  test/.style={base, diamond, aspect=2, text width=10em},
  term/.style={proc, align=center, rounded corners},
  % coord node style is used for placing corners of connecting lines
  coord/.style={coordinate, on chain, on grid, node distance=25mm and 60mm},
  % nmark node style is used for coordinate debugging marks
  nmark/.style={draw, cyan, circle, font={\sffamily\bfseries}},
  % -------------------------------------------------
  % Connector line styles for different parts of the diagram
  norm/.style={->, draw},
  free/.style={->, draw, lcfree},
  cong/.style={->, draw, lccong},
  it/.style={font={\small\itshape}}
}

\node [term, join] (p0) {Procedure to pack the ROI's of an image to form a lower sized image};
\node [proc, join] (p1) {Find all connected components in a graph where the nodes are the bounding boxes of the ROI's and two nodes are connected if the corresponding bounding boxes intersect};
\node [proc, join] (p2) {Find the enclosing bounding box around the union of bounding boxes in each connected component and form new set of bounding boxes.};
\node [test, join] (p3) {Do the new set of bounding boxes intersect?};
\node [proc] (p4) {Decide on the layout of the bounding boxes in the lower sized output image};
\node [proc,join] (p5) {Check which pairs of bounding boxes can potentially intersect when expanded in either the horizontal or vertical direction.};
\node [proc,join] (p6) {Decide whether to extend horizontally or vertically first};
\node [proc,join] (p7) {Extend the bounding boxes simultaneously in each dimension in order until the lower sized output is completely filled in that dimension or the bounding boxes start intersecting with each other};
\node [proc,join] (p8) {Extract patches from the original image according to the final bounding boxes and place them in the lower sized image according to the decided layout};
\node [coord, left=of p3]  (c4)  {};  

\path (p3.south) to node [near start, xshift=1em] {$No$} (p4);
  \draw [*->] (p3.south) -- (p4);v 
\path (p3.west) to node [yshift=-1em] {$Yes$} (c4); 
  \draw [*->] (p3.west) -- (c4) |- (p1); 
\end{tikzpicture}
\caption{Flowchart illustrating the overall flow of the ROI packing algorithm. Please refer to figure \ref{fig:illustration} to observe the results of the ROI packing algorithm} \label{fig:flow1}
\end{figure*}
\par
\begin{figure*}
  \centering
\begin{tikzpicture}[%
    >=triangle 60,              % Nice arrows; your taste may be different
    start chain=going below,    % General flow is top-to-bottom
    node distance=8mm and 45mm,>=latex]
 \tikzset{
   base1/.style={draw, on chain, on grid, align=center, minimum height=5ex},
   proc1/.style={base1, rectangle, text width=8em},
   proc2/.style={base1, rectangle, text width=30em},
   proc3/.style={base1, rectangle, text width=15em},
   root/.style={base1, rectangle, text width=15em},
   test1/.style={base1, diamond, align=center, text width=7em},
   term1/.style={proc2, align=center, rounded corners}
   }
\node [term1] (p0) {Procedure to decide the layout of the image and whether to extend each bounding box horizontally or vertically first.};
\node [test1] (p1) {Is the largest dimension of all the bounding boxes height of a bounding box?};
\node [proc1,right= of p1] (p2) {Similar set of steps as the yes condition (Symmetrically opposite)};
\node [proc2,below of = p1,yshift=-20mm] (p3) {Decide to extend all bounding boxes horizontally first};
\node [root,below of = p3] (p4) {switch(no. of bounding boxes)};
\node[proc1,below of = p4,xshift=-50mm,yshift=-40mm] (c1) {Single BBOX fills the entire image};
\node[proc1,below of = p4, xshift = -17mm,yshift=-40mm] (c2) {Place the 2 BBOX's horizontally by their side};
\node[proc1,below of = p4, xshift = 17mm,yshift=-40mm] (c3) {The BBOX with the largest height is placed in a separate column and the other two bounding boxes are placed vertically stacked horizontal to the first BBOX};
\node[proc1,below of = p4, xshift = 50mm,yshift=-40mm] (c4) {BBOX with the largest height and 3rd largest height are placed in the first column stacked vertically. BBOX's with 2nd largest and 4th largest height are placed in the second column stacked vertically.};
\path (p0.south) to node [near start, xshift=1em] {} (p1);
  \draw [->] (p0.south) -- (p1); 
\path (p1.east) to node [near start, xshift=0.3em, yshift=1em] {$No$} (p2);
  \draw [*->] (p1.east) -- (p2); 
\path (p1.south) to node [near start, xshift=1.2em] {$Yes$} (p3);
  \draw [*->] (p1.south) -- (p3);
\path (p3.south) to node [near start, xshift=1em] {} (p4);
  \draw [->] (p3.south) -- (p4);
\path (p4.south) to node [near start, xshift=0.3em] {$1$} (c1);
  \draw [->] (p4.south) -- (c1);
\path (p4.south) to node [near start, xshift=0.3em] {$2$} (c2);
  \draw [->] (p4.south) -- (c2);
\path (p4.south) to node [near start, xshift=0.3em] {$3$} (c3);
  \draw [->] (p4.south) -- (c3);
\path (p4.south) to node [near start, xshift=0.3em] {$4$} (c4);
  \draw [->] (p4.south) -- (c4);
\end{tikzpicture}
  \caption{Flowchart detailing the layout procedure. Please refer to figure \ref{fig:illustration} to observe the results of the layout procedure. The cases with 1,2 and 4 non-overlapping bounding boxes have been illustrated in figure \ref{fig:illustration}}
  \label{fig:tiling}
\end{figure*}
\section{Experimental Methodology}
\label{sec:experiment}
The ImageNet object detection dataset (DET) is a dataset comprising 200 classes of objects which is a subset of the ImageNet 1000 classes. Further, the ImageNet video object detection dataset (VID) comprises of 30 classes of objects which is a subset of the DET 200 classes. The ImageNet video object detection (VID) dataset was the most appropriate choice for illustrating the results of our work. The ImageNet VID training set has 3862 video snippets and the ImageNet VID validation set has 555 video snippets. 53539 frames from the DET dataset comprising only of the classes from the VID dataset and 57834 frames from the VID training set were combined to form the final training set. 
%This information is summarized in figure \ref{tab:dataset}. 
\par 
The SSD300 \cite{liu2016ssd} object detector operated on a per-frame basis was used as the baseline for our work. The SSD300 object detector uses VGG16 as feature extractor. The SSD300 pretrained model on the DET dataset was further trained on our training set for 210k iterations with a learning rate of $10^{-3}$ for the first $80000$ iterations, $10^{-4}$ for the next $40000$ iterations and $10^{-5}$ for the rest of the training. This SSD300 trained model gave a mAP score of $70.6$ on the VID validation set. Further, this model has a network throughput of $47$ fps and a overall throughput (including standard pre-processing time) of $18$ fps.
%\par
%\begin{figure}
%\begin{centering}
%\begin{tabular}{|p {2cm}|p {1cm} |p {1cm} |p {1cm} |}
%\hline 
%Dataset & No. of classes & No. of video snippets & No. of frames selected\tabularnewline
%\hline 
%\hline 
%DET training set & 200 & N/A & 53539\tabularnewline
%\hline 
%VID training set & 30 & 3862 & 57834\tabularnewline
%\hline 
%VID validation set & 30 & 555 & 176126\tabularnewline
%\hline 
%\end{tabular}\caption{Details of the ImageNet DET and ImageNet VID dataset}\label{tab:dataset}
%\par\end{centering}
%\end{figure}
One might suppose that we need two object detectors for our framework - one for higher sized images and one for lower sized images. The SSD300 network processes images at $300\times300$ as the name suggests. However, closer observation of the network suggested that the same network can process $150\times150$ images as well by stopping processing at the penultimate layer. Hence, we use the same SSD300 network with the same weights to process both higher sized images and lower sized images. In all our experiments, the baseline size $s_{1}$ is $300$ and the final lower size $s_{3}$ is $150$. When a $150\times150$ sized image is passed on to the SSD300 network, processing is configured to stop at the penultimate layer. All the experiments were performed using the SSD Caffe framework in a 2.1 GHz Intel Xeon CPU with a  Nvidia TITAN X GPU. Code will be released soon. In all the experiments, the batch size was $1$ to emulate an online setup. The detection threshold $\tau$ used to select ROIs was fixed at $0.2$ in most of our experiments unless explicitly specified otherwise.
\section{Experimental Results}
\label{sec:results}
\subsection*{Results from sample videos}
We show results on processing some sample videos with PaD. In figure \ref{fig:illustration}, we show some sample detections with our ROI-packing algorithm. The first column shows frame $i$. The second column shows the ROI packed frame $i+1$ with the detections. The third column shows the original frame $i+1$ with detections transformed from ROI packed frame $i+1$. For this experiment, the confidence threshold $\tau$ for selecting a detection as an ROI for the next frame is chosen as $0.3$ for the sake of illustration. All bounding boxes with a minimum threshold of $0.2$ are shown in the figure.
\begin{figure*}
\centering
%\advance\leftskip-3cm
%\advance\rightskip-3cm
\begin{tabular}{c|c|c}
Frame $i$ & ROI-packed frame $i+1$ & Frame $i+1$\\
\hline
\subfloat{\includegraphics[scale=0.15]{image1.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image2.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image3.JPEG}} \\[-0.3in]

\subfloat{\includegraphics[scale=0.15]{image4.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image5.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image6.JPEG}} \\[-0.3in]

\subfloat{\includegraphics[scale=0.15]{image7.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image8.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image9.JPEG}} \\[-0.3in]

\subfloat{\includegraphics[scale=0.15]{image10.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image11.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image12.JPEG}} \\

\end{tabular}
\caption{Sample set of consecutive frames processed with the ROI packing mechanism. The first column shows frame $i$. The second column shows the ROI packed frame $i+1$ with the detections. The third column shows the original frame $i+1$ with detections transformed from ROI packed frame $i+1$. For this experiment, the confidence threshold for selecting a detection as an ROI for the next frame is chosen as $0.3$ for the sake of illustration. All bounding boxes with a minimum threshold of $0.2$ are shown in the figure.}
\label{fig:illustration}
\end{figure*}
\par
In figures \ref{fig:tt}(a), we plot the time taken per frame for processing a sample video and the cumulative time taken for processing the same video using PaD and compare it with the baseline. It can be seen that processing the lower sized frame of $150\times150$ is almost $3\times$ faster. When ROI-packing fails, there is a slight overhead incurred which is visible towards the end of the video in figure \ref{fig:tt}(a). Also, we see that some frames require almost $0$s for processing. This is because the previous frame had no detections. Overall, we note that processing the video using PaD requires almost $8$s lesser time than the baseline from figure \ref{fig:tt}(b).
\begin{figure*}
  \centering
  \begin{tabular}{cc}
  \subfloat[]{\includegraphics[scale=0.4]{Videoprocess1_arrow.png}} &
\subfloat[]{\includegraphics[scale=0.35]{Videoprocess2.png}} \\
  \end{tabular}
  \caption{(a)Time taken per frame for processing a sample video (b)Cumulative time taken processing a sample video}
  \label{fig:tt}
\end{figure*}

\subsection*{Results over the entire dataset}
PaD was run with a inter-anchor distance $d=5$ and $s_{2}=150$. In figure \ref{fig:tpvpf}, we plot the histogram of average per-frame processing time on a video-by-video basis. In other words, the average time taken per frame was obtained for each video and is plotted as a histogram. From the figure, we can clearly see that the average time taken to process a frame is lower using PaD for more videos than the baseline. The baseline mAP score is $70.6$ and our method has a mAP score of $69.5$. Thus the mAP score drops by less than $1.6\%$ and $1.1$ percentage points. The average per-frame speedup is around $1.25 \times$. The average overhead incurred for ROI-packing is around $9\%$ of the total time taken.
\begin{figure}
  \centering
  \includegraphics[scale=0.4]{tpvpf_hist.png}
  \caption{Histogram of average per-frame processing time on a video-by-video basis}
  \label{fig:tpvpf}
\end{figure}
\subsection*{Comparison with a naive ROI-packing algorithm}
In order to illustrate the benefits of our sophisticated ROI-packing algorithm discussed in section \ref{sec:Methodology}, we compare the accuracy drop when compared with a naive ROI-packing algorithm.
\par
The naive ROI-packing algorithm works as follows. The naive ROI-packing algorithm can accommodate upto four ROI's just like the sophisticated method. If there are more than four objects in the frame, the frame is processed at full size. Otherwise, the bounding box surrounding each frame is extended by a factor of $1.2\times$ and is treated as an ROI. If there is only one object, the ROI surrounding the bounding box is rescaled to size $s_{3} \times s_{3}$ and is processed by the detector. If there are two objects, the lower sized frame is divided into two columns of size $s_{3} \times \frac{s_{3}}{2}$. The two ROIs are rescaled to the appropriate sizes and laid out on the lower sized frame. In the case of three or four objects, the lower sized frame is divided into four regions in two columns and two rows of size $\frac{s_{3}}{2} \times \frac{s_{3}}{2}$. In the case of three ROIs, the ROIs will be rescaled to occupy three of the four regions in the frame and the fourth region will be left blank. In the case four ROIs, the ROIs will be rescaled and fit to these four regions. We do not perform a greedy expansion of the RoIs to provide background context. Instead, the ROIs are just expanded by a constant factor of $1.2 \times$ and rescaled to appropriate size.
\par
Our sophisticated ROI packing method with inter-anchor distance $d=5$ gave a mAP score of $69.5$. With the same parameter setting, the naive ROI packing algorithm gave a mAP score of $56.8$. This clearly illustrates the need for a sophisticated ROI packing algorithm that preserves the scale and aspect ratio of the ROIs and provides as much background context as possible. Further, each object should be present in only one ROI to prevent redundant detections. This clearly shows that the CNN object detectors, though fairly robust to small scale changes cannot handle large variations in scale and are particularly sensitive to the aspect ratio. Also, CNN object detectors are overfit to the background context.
\subsection*{Tradeoff between speed and accuracy by parameter variation}
In figure \ref{fig:tradeoff1}, we vary the inter-anchor distance $d$  with $s_{2}=150$ and observe the effect on mAP score and speed. As $d$ is varied from $2$ to $10$, the mAP drops from $70.1$ to $68.9$ while the FLOP count reduction relative to the baseline increases from $18\%$ to $39\%$ on average over the entire validation set. Thus, the inter-anchor distance can be tuned according to the speed-accuracy tradeoff desired.
\begin{figure*}
  \centering
  \begin{tabular}{cc}
  \subfloat{\includegraphics[scale=0.3]{map_iad.png}} &
\subfloat{\includegraphics[scale=0.3]{speed_iad.png}} \\
  \end{tabular}
  \caption{Figure depicting the speed-accuracy tradeoff achieved by varying the inter-anchor distance}
  \label{fig:tradeoff1}
\end{figure*}
\par
The parameters $s_{1}=300$ and $s_{3}=150$ are decided by the specific CNN detector that is being used. However, the factor $s_{2}$ could be varied to obtain higher speeds. As $s_{2}$ is increased, the chances of the ROIs fitting in the lower sized layout increases, which in turn increases the chances of processing the frame at lower size. The speed-accuracy tradeoff with variation in $s_{2}$ is plotted in figure \ref{fig:tradeoff2}. With increase in $s_{2}$ from $150$ to $200$, the average FLOP count reduction relative to the baseline varies from $32\%$ to $44\%$. The average per-frame speedup increases from $1.21\times$ to $1.33\times$. However, there is relatively a high drop in accuracy to $6\%$ relative to the baseline at $s_{2}=200$. This shows that the CNN object detector though fairly robust to scale variations cannot handle large variations in scale.
\begin{figure*}
  \centering
  \begin{tabular}{cc}
  \subfloat{\includegraphics[scale=0.3]{map_scale.png}} &
\subfloat{\includegraphics[scale=0.3]{speed_scale.png}} \\
  \end{tabular}
  \caption{Figure depicting the speed-accuracy tradeoff achieved by varying the scaling factor}
  \label{fig:tradeoff2}
\end{figure*}
\section{Conclusion and Future Work}
\label{sec:conclusion}
Still-image object detection has improved by leaps and bounds in recent years due to the success in training and deploying neural networks. However, the opportunities that are available in the context of videos have not been fully exploited. Neural networks are in general very compute-hungry and inference can run in real-time in only the most high-end GPUs. In this work, we use the opportunities available in the context of videos to speed up and reduce the amount of computation in neural network object detectors. In PaD, the full-sized input will only be processed in anchor frames. In the inter-anchor frames, the ROIs in the frame are identified based on the location of the objects in the previous frame. These ROIs are packed together in a lower sized frame which is fed to the CNN object detector. The ROI packing algorithm needs to be sophisticated in the sense that it has to ensure that the scales and aspect ratios of the objects are preserved and enough background context is provided. With this setup, we observed $1.25 \times$ speedup with less than $1.6\%$ drop in accuracy on the ImageNet VID validation set. Further, the time taken to process a lower sized frame is almost $3 \times$ lesser and the FLOP count reduces by $4 \times$. Given more suitable datasets, we can get even more speedup and reduction in FLOP count in the average sense.
\par
As part of future work, we plan to incorporate a motion model to obtain the ROIs in the current frame. Incorporating a motion model could also help extend this framework to larger batch sizes. Also, it is possible to use two different models or networks to process larger sized and smaller sized frames. This will help reduce the accuracy drop but will in turn increase the memory footprint. There is an overhead incurred in checking whether the ROIs can fit in the lower sized frame. Currently, we select anchor frames at regular intervals. However, information on whether ROIs were packed successfully in previous frames can help us decide how frequently we select anchor frames. Thus, another line of future work is a dynamic mechanism for selecting anchor frames in order to reduce the overhead. Further, instead of using a heuristic hand-crafted algorithm for forming the ROI packed frame, a neural network could be trained to identify the ROIs and pack them in a lower sized frame like in an attention mechanism. This is another ambitious line of future work. It would be interesting to test PaD in more resource constrained platforms like mobile GPUs and CPUs. We expect the benefits to be more pronounced in such platforms.  

==> Athindran_body2.tex <==
\section{Introduction}
The task of object detection in videos \cite{KangTCNN16,zhu2017deep,Kang_2016_CVPR,Kang2017object,zhu2017flow,Zhu_2018_CVPR,TSSD,pan2018recurrent,mobilevideo,fastYOLO} has been gaining attention in recent years. It can serve as an important preprocessing task primarily for object tracking and for several other video processing tasks such as video summarization and video search. Further, object detection and tracking can aid  various important applications such as traffic monitoring, pedestrian tracking, animal monitoring and environment survey using drones. Many of these applications require video frames to be processed in real-time in resource-constrained environments. It is thus imperative to design systems that can detect objects in videos in a fast, compute-light and accurate manner.
\par
 Still-image object detection has been studied extensively in the past. The accuracy and speed of still-image object detection have improved by leaps and bounds in recent years due to innovations in the usage of deep convolutional neural networks (CNN) for object detection. The state-of-the-art CNN based still-image object detectors currently are faster RCNN \cite{NIPS2015_FRCNN}, SSD \cite{liu2016ssd}, YOLO \cite{CVPR_YOLO,yolo9000,yolov3} and RFCN\cite{dai2016r}. SSD and YOLO are almost $7-10 \times$ faster than faster-RCNN and RFCN and give comparable accuracy (mAP score) on standard still-image object detection datasets. 
\par
These still-image object detectors can be extended for object detection in videos by using them on a per-frame basis. However, this is inefficient as there is a strong temporal correlation between frames in a video. This temporal redundancy can be leveraged either to improve the accuracy or speed of object detection. In the recent past, there have been several attempts to improve the accuracy of object detection in videos by either integrating the bounding boxes \cite{KangTCNN16,Kang_2016_CVPR,han2016seq,penglinking} or features \cite{Kang2017object,zhu2017flow,Zhu_2018_CVPR,hetangimpression} across frames. However, there has not been enough attention on leveraging this temporal redundancy to improve speed. Some exceptions to this norm are \cite{zhu2017deep,TSSD,pan2018recurrent,mobilevideo,fastYOLO}. In this work, we propose a method, Pack and Detect (PaD), for fast object detection in videos with negligible loss in accuracy.
\par
Neural networks are in general very computationally intensive. For example, processing a video at $300 \times 300$ resolution using the SSD300 (Single Shot Detector) object detection network with VGG16 as backbone at 30 fps requires 1.87 trillion FLOPS/s. Several attempts \cite{szesurvey} have been made to make them less compute-hungry. Techniques such as pruning weights or connections \cite{HanMD15,Han2015}, pruning filters in full or part in a CNN \cite{thinet,NIPS2016_ssparsity,Guo2017,deepakrandom,haopruning}, reducing the precision of floating point operations \cite{AxNNvenkat,anwarprecision} and designing compute-light architectures \cite{mobilenet,squeezenet} have proven to be successful in the past. While most of these methods are static and are employed at design time, there are some methods such as conditional computation \cite{bengiocondcomp}, dynamic deep neural networks (D2NN) \cite{LiuD17} and dynamic variable effort deep neural networks \cite{GanapathyVRR17} (DyVEDEEP) that dynamically adjust the amount of computation to be employed for an input. However, firstly, all of these methods do not exploit the specific opportunities that can be leveraged in the context of videos. Secondly, all of these methods try to modify the network and do not try to compress the inputs to be fed into the network.
\par
In particular, there are two opportunities we are trying to leverage in the context of videos. Firstly, the objects of interest have been observed to occupy only a small fraction of the area in an image. Secondly, there is a strong temporal correlation between frames in a video. We propose Pack and Detect (PaD) which leverages these two opportunities. The full-sized image is only processed in selected frames called anchor frames. In the frames between the anchor frames (inter-anchor frames), the detections from the previous frame are used to identify regions in the image where an object could potentially be located. These regions are called regions of interest (ROIs). The ROIs are packed in a lower sized image which is fed into the detector.
\par 
We propose a ROI packing algorithm based on a greedy heuristic that is responsible for packing the ROI's in the lower-sized frame while meeting the following criteria:
\begin{enumerate}
\item Each ROI is expanded to provide as much background context as possible to maintain the accuracy of the detector.
\item There is minimal loss of resolution and no change in aspect ratio to maintain the accuracy of the detector.
\item Each object is present in an unique ROI. 
\item The space in the lower-sized frame is used as efficiently and impartially as possible.
\end{enumerate}
\par
Our method, PaD,  which uses the ROI-packing algorithm to compress the input in inter-anchor frames is naturally faster because of the smaller size of the input fed to the object detector. In the inter-anchor frames, the FLOP count can potentially reduce by a factor of $4\times$. Tuning the algorithm parameters can provide a $1.3\times$ increase in throughput with only a $2.5\%$ drop in accuracy compared to a baseline mechanism that uses the object detector on a per-frame basis. We vary different parameters of the algorithm to achieve a tradeoff between speed and accuracy. Further, we present results that provide insight into the inner workings of the algorithm. 
\par
In section \ref{sec:rel_work}, we review some of the related work. In section \ref{sec:motivation}, we analyze the two opportunities we are trying to leverage in the context of videos. In section \ref{sec:Methodology}, we provide a overview of the methods and algorithms used in our work. Section \ref{sec:experiment} outlines the experimental methodology and section \ref{sec:results} reports the results obtained from our experiments. In section \ref{sec:conclusion}, we conclude our work.

\section{Related Work}
\label{sec:rel_work}
\subsection*{Object Detection in Videos}
The temporal redundancy in videos has been exploited before to improve the accuracy and speed of object detection in videos. In \cite{KangTCNN16,Kang_2016_CVPR,han2016seq,penglinking}, the aggregation of information from neighbouring frames is done at the bounding box level to improve accuracy. In \cite{KangTCNN16}, per-frame object detection is combined with multi-context suppression, motion-guided propagation and object tracking to improve detection accuracy. In \cite{han2016seq,penglinking}, non-maximum suppression is done over bags of frames. In \cite{Kang2017object,zhu2017flow,Zhu_2018_CVPR,hetangimpression}, there is integration of the CNN features across neighbouring frames to improve accuracy. In \cite{Kang2017object}, a CNN is combined with a LSTM (Long Short Term Memory) to obtain temporal features for object detection. In \cite{zhu2017flow, Zhu_2018_CVPR,hetangimpression}, the features from neighbouring frames are aggregated together using optical flow information to improve feature quality. All the methods discussed till now are extremely slow and \cite{KangTCNN16,Kang_2016_CVPR,han2016seq,penglinking,Kang2017object} are not online.
\par
On the other hand, \cite{zhu2017deep,TSSD,pan2018recurrent,mobilevideo,fastYOLO} are relatively faster methods aimed at object detection in a video. The methods in \cite{TSSD,mobilevideo,fastYOLO} are faster by virtue of using a faster still-image object detector or an efficient backbone network. In \cite{zhu2017deep}, the feature maps of the CNN are not computed in all the frames. The feature maps from anchor frames are transferred to neighbouring frames by warping them with optical flow information. Since the features are not recomputed in each frame, this setup is much more faster and compute-efficient. In \cite{pan2018recurrent}, neighbouring frames are subtracted to give rise to a sparse input. This sparse input is processed by the CNN with the EIE \cite{Han2016} hardware accelerator to achieve computational savings. The methods proposed in this paper are vastly different than the methods in the literature to speed-up video object detection. Even though the overall speed-up achieved in an average sense in our work might not be as high as the $5\times$ reported in \cite{zhu2017deep}, PaD can be used alongside the methods in \cite{zhu2017deep} using some simple tricks to increase the efficiency further. Any efficient neural network or faster object detector can be used with PaD as in \cite{TSSD,mobilevideo,fastYOLO} to obtain further speed-up. Finally, PaD does not require any specialized hardware accelerator like in \cite{pan2018recurrent} to obtain computational savings.
\subsection*{Efficient Neural Networks}
There have been efforts to reduce the number of computations of neural networks using various techniques. Deep compression \cite{HanMD15} deployed on a custom hardware accelator\cite{Han2016} can result in considerable amount of savings in computation and speedup for standard neural networks. Deep compression works by pruning weights less than a threshold, quantizing the weights using clustering followed by huffman coding. EIE \cite{Han2016} is an hardware accelerator that can leverage the sparsity of the deep compressed DNN to speed up the network. Since, fine-grained sparsity has not been shown to improve the speed without custom hardware accelerators, there have been techniques to induce structured sparsity\cite{NIPS2016_ssparsity} by pruning filters \cite{thinet,NIPS2016_ssparsity,Guo2017,deepakrandom,haopruning} of a CNN in full or part. MobileNet\cite{mobilenet} replaces the standard convolution with a combination of depth-wise and point-wise convolution to reduce computation. SqueezeNet\cite{squeezenet} utilizes CNN design techniques to reduce the number of computations and memory. Another innovation is the concept of Big-Little neural networks \cite{biglittle} that first try to use a smaller network to process the image. If the little network is not capable of successfully achieving its task in the frame, the bigger network is used to process the image. This method has been shown to reduce computation significantly without much loss in accuracy.
\par
Most of the methods for achieving computational efficiency in neural networks are static methods to be employed at design time. However, there are some exceptions. Conditional computation \cite{bengiocondcomp} selectively activates certain parts of the network depending on the input. The policy for deciding which parts of the network to activate is learnt using reinforcement learning. Dynamic deep neural networks (D2NN) \cite{LiuD17} work in a manner similar to conditional computation and turn on/off regions of the network using reinforcement learning. DyVEDEEP \cite{GanapathyVRR17} is an unique effort to reduce the computations in neural networks dynamically by using three strategies - saturation prediction and early termination, significance driven selective sampling and similarity-based feature map approximation. 
\par
All the methods try to compress or tweak the model/network to reduce computations and achieve speedup. In this work, we compress the inputs that we feed into the network. Hence, PaD is orthogonal to most existing techniques and can be used in combination with other methods.
\subsection*{Visual Attention Mechanism}
Inspired by human vision, there have been several attempts \cite{NIPS2010_4089,Ranzato14,Mnih2014,ba2014multiple,kosiorek2017hierarchical,kahou2015ratm} to reduce computation by processing an image as a sequence of glimpses rather than processing the image as a whole. The notion of a foveal glimpse is somewhat similar to the idea of ROI discussed here. However, there are several important differences. A foveal glimpse is a high resolution crop of an important region in the image that is crucial to the task at hand. In our work, we pack all the ROIs together in a single frame and do not process them sequentially like how glimpses are processed. Further, the most important difference is that the location of ROI's is inferred from the detections in the previous frame in a video and the network does not need to learn where to look through an attention mechanism. Also, a foveal glimpse obtains crops by extracting pixels close to the location target at high resolution and pixels far from the location target at low resolution. We do not do any multi-resolution processing in our work. Hence, our work, though somewhat inspired from the notion of foveal glimpse is considerably different. 
\section{Motivation}
\label{sec:motivation}
\subsection{Occupancy of objects in a image}
In this work, an opportunity that we try to leverage is the fact that most of the pixels in a frame are clutter and the objects of interest occupy only a small fraction of an area in the frame. We back this hypothesis using statistics from a popular video dataset. From a analysis of the ImageNet VID validation set containing $555$ videos with $176126$ frames, we see that the objects occupy only $22.7\%$ of the image on the average. Figure \ref{fig:occupancy} is a histogram of the object occupancy ratio statistics in the dataset. From the figure, we can infer that the in a huge majority of the frames, the objects occupy less than $30\%$ of the area in a frame.
\begin{figure}
  \centering
  \includegraphics[scale=0.4]{ratios_hist.png}
  \caption{Histogram of object occupancy ratio}
  \label{fig:occupancy}
\end{figure}

\subsection{Temporal correlation of object locations in a video}
In general, we can expect a lot of temporal correlation between consecutive frames in a video unless there are sudden camera shifts or missing frames. We observe this hypothesis to be true from a statistical analysis of the ImageNet VID validation set. On the average, the IoU of area containing objects between consecutive frames is $94.4\%$. Figure \ref{fig:ROIoverlap} is a histogram of the object occupancy area IoU statistics between consecutive frames in the dataset. In the figure we can clearly see a sharp peak close to $1$. We exploit this opportunity in our work.
\begin{figure}
  \centering
  \includegraphics[scale=0.4]{ious_hist.png}
  \caption{Histogram of IoU of regions containing objects between consecutive frames}
  \label{fig:ROIoverlap}
\end{figure}
\section{Methodology}
\label{sec:Methodology}
\subsection{Architecture}
The overall architecture of the methodology proposed in this work is presented in figure \ref{fig:arch}. Full-sized video frames are processed at regular intervals (inter-anchor distance $d$). In the other frames, the ROIs are identified based on the locations of the detections from the previous frame. Only detections with a minimum confidence threshold $\tau$ are taken into consideration. ROI is a region which is likely to contain an object. An ROI packing algorithm will try to pack the ROIs in a lower sized frame. If the packing is successful, then the lower sized frame is processed instead, giving rise to computational savings. However, if the packing is not successful, then the frame is processed at full size. Hence, there is an overhead of checking whether ROI packing is possible. Once the lower sized ROI-packed frame is processed using the CNN detector, the object detections in the ROI packed frame have to be transformed to the original frame dimensions. This can easily be done by keeping track of the ROI boundaries in the original frame.
\begin{figure*}
\centering
\begin{tikzpicture}[auto, node distance=2.5cm and 4 cm,>=latex]
\tikzset{
  base/.style={draw, on grid,align=center, minimum height=8ex},
  proc/.style={base, rectangle, text width=6em},
  test/.style={base, diamond, text width=4em},
  coord/.style={coordinate, on grid},
}
\node[test,xshift=40mm](p0){\tiny Is frame anchor frame?};
\node[proc,below of = p0](p1){\tiny Process frame at full size};
\node[proc,right of = p0](p2){\tiny Infer the ROI's in the frame based on the detections from the previous frame};
\node[proc,right of = p2](p3){\tiny Run the ROI packing algorithm to pack the ROI's in a lower sized frame};
\node[test, right of = p3](p4){\tiny Is ROI packing successful?};
\node[proc, below of = p4](p5){\tiny Process frame at lower size};
\path (p0.south) to node [near start, xshift=0.2em] {$Yes$} (p1);
\draw [*->] (p0.south) -- (p1);
\path (p0.east) to node [near start, xshift=0.2em] {$No$} (p2);
\draw [*->] (p0.east) -- (p2);
\path (p2.east) to node [near start, xshift=0.2em] {} (p3);
\draw [->] (p2.east) -- (p3);
\path (p3.east) to node [near start, xshift=0.2em] {} (p4);
\draw [->] (p3.east) -- (p4);
\path (p4.south) to node [near start, xshift=0.2em] {$Yes$} (p5);
\draw [*->] (p4.south) -- (p5);
\node [coord, above of = p4, yshift=-1em]  (c1)  {};
\node [coord, left of = p1, node distance = 6em] (c2){};
\path (p4.north) to node [xshift=2em] {$No$} (c1);
  \draw [*-] (p4.north) -- (c1) -| (c2);
\path (c2.east) to node [xshift=1em]{}(p1);
  \draw [->] (c2.east) -- (p1);   
\end{tikzpicture}
\caption{Overall Architecture of PaD} \label{fig:arch}
\end{figure*}

\subsection{ROI packing algorithm}
In figure \ref{fig:flow1}, we illustrate the overall flow of our ROI packing algorithm based on a greedy heuristic. This algorithm is key to ensure that there is no significant drop in accuracy due to ROI packing. As a first step in the algorithm, we find all the connected components of all nodes in a graph where nodes represent ROIs and two nodes are connected if their respective ROI's intersect. We then find the enclosing bounding box over the union of ROI's in each connected component. We iterate the connected components algorithm until we ensure that none of the final bounding boxes overlap. This constraint is important because if two bounding boxes overlap, then parts of the same object could be present two or more times in the ROI packed frame.
\par
Once the number and size of the bounding boxes are decided, the layout of the bounding boxes is determined by a heuristic procedure. The flowchart in figure \ref{fig:tiling} illustrates the algorithm used for determining the layout. Simpler variants of this procedure could also be adopted. Once the layout is decided, a check is done to see whether the bounding boxes can fit in the layout. If it is not possible to fit the bounding boxes in the layout, the ROI packing procedure stops here and the image is processed at full size.
\par 
If the bounding boxes can be fit in the layout, the following procedure is carried out. Using experiments, we noted that CNN object detectors are often overfit to the background context of the object to be detected. The performance of the CNN object detector is poor if there is no background context. Hence, we extend each bounding box within the space available for each bounding box in the layout to provide as much context as possible to the CNN detector. The algorithm for extending the bounding boxes works as follows. First, we make a decision using some heuristic rules as to whether to extend the boxes horizontally or vertically first. For the sake of discussion, let us assume that the choice is to extend horizontally all the bounding boxes first. We find all the bounding boxes, which could potentially intersect when extended horizontally. We extend all bounding boxes horizontally until the layout size is reached or the bounding boxes start intersecting with each other. Then we repeat the same procedure in the other dimension. Once the final bounding boxes are decided, the corresponding regions in the image are extracted and the lower sized frame is filled according to the decided layout.
\par
There are a lot of heuristic rules in the ROI packing algorithm. All of these rules have been decided after thorough analysis of the setup using experiments. In section \ref{sec:results}, we show some results illustrating that this sophisticated ROI packing algorithm is superior to a naive ROI packing algorithm. Further, there are two parameters we can tune to achieve a speed-accuracy tradeoff. Firstly, an obvious parameter that can be tuned is the inter-anchor distance $d$. Also, most of the CNN object detectors have some amount of robustness inbuilt to tackle scale variations. Hence, we could fit the ROI's extracted from a $s_{1} \times s_{1}$ sized frame into a $s_{2} \times s_{2}$ frame and downscale the ROI packed frame to $s_{3} \times s_{3}$ to get higher speed-ups. There will be some loss of accuracy due to the downscaling. We explore these trade-offs in section \ref{sec:results}.
\begin{figure*}
\centering
\begin{tikzpicture}[%
    >=triangle 60,              % Nice arrows; your taste may be different
    start chain=going below,    % General flow is top-to-bottom
    node distance=6mm and 60mm, % Global setup of box spacing
    every join/.style={norm},   % Default linetype for connecting boxes
    ]
\tikzset{
  base/.style={draw, on chain, on grid, align=center, minimum height=1ex},
  proc/.style={base, rectangle, text width=30em},
  test/.style={base, diamond, aspect=2, text width=10em},
  term/.style={proc, align=center, rounded corners},
  % coord node style is used for placing corners of connecting lines
  coord/.style={coordinate, on chain, on grid, node distance=25mm and 60mm},
  % nmark node style is used for coordinate debugging marks
  nmark/.style={draw, cyan, circle, font={\sffamily\bfseries}},
  % -------------------------------------------------
  % Connector line styles for different parts of the diagram
  norm/.style={->, draw},
  free/.style={->, draw, lcfree},
  cong/.style={->, draw, lccong},
  it/.style={font={\small\itshape}}
}

\node [term, join] (p0) {\tiny Procedure to pack the ROI's of an image to form a lower sized image};
\node [proc, join] (p1) {\tiny Find all connected components in a graph where the nodes are the bounding boxes of the ROI's and two nodes are connected if the corresponding bounding boxes intersect};
\node [proc, join] (p2) {\tiny Find the enclosing bounding box around the union of bounding boxes in each connected component and form new set of bounding boxes.};
\node [test, join] (p3) {\tiny Do the new set of bounding boxes intersect?};
\node [proc] (p4) {\tiny Decide on the layout of the bounding boxes in the lower sized output image};
\node [proc,join] (p5) {\tiny Check which pairs of bounding boxes can potentially intersect when expanded in either the horizontal or vertical direction.};
\node [proc,join] (p6) {\tiny Decide whether to extend horizontally or vertically first};
\node [proc,join] (p7) {\tiny Extend the bounding boxes simultaneously in each dimension in order until the lower sized output is completely filled in that dimension or the bounding boxes start intersecting with each other};
\node [proc,join] (p8) {\tiny Extract patches from the original image according to the final bounding boxes and place them in the lower sized image according to the decided layout};
\node [coord, left=of p3]  (c4)  {};  

\path (p3.south) to node [near start, xshift=1em] {\tiny $No$} (p4);
  \draw [*->] (p3.south) -- (p4);v 
\path (p3.west) to node [yshift=-1em] {\tiny $Yes$} (c4); 
  \draw [*->] (p3.west) -- (c4) |- (p1); 
\end{tikzpicture}
\caption{Flowchart illustrating the overall flow of the ROI packing algorithm. Please refer to figure \ref{fig:illustration} to observe the results of the ROI packing algorithm} \label{fig:flow1}
\end{figure*}
\par
\begin{figure*}
  \centering
\begin{tikzpicture}[%
    >=triangle 60,              % Nice arrows; your taste may be different
    start chain=going below,    % General flow is top-to-bottom
    node distance=5mm and 45mm,>=latex]
 \tikzset{
   base1/.style={draw, on chain, on grid, align=center, minimum height=1ex},
   proc1/.style={base1, rectangle, text width=8em},
   proc2/.style={base1, rectangle, text width=30em},
   proc3/.style={base1, rectangle, text width=15em},
   root/.style={base1, rectangle, text width=15em},
   test1/.style={base1, diamond, align=center, text width=7em},
   term1/.style={proc2, align=center, rounded corners}
   }
\node [term1] (p0) {\tiny Procedure to decide the layout of the image and whether to extend each bounding box horizontally or vertically first.};
\node [test1] (p1) {\tiny Is the largest dimension of all the bounding boxes height of a bounding box?};
\node [proc1,right= of p1] (p2) {\tiny Similar set of steps as the yes condition (Symmetrically opposite)};
\node [proc2,below of = p1,yshift=-20mm] (p3) {\tiny Decide to extend all bounding boxes horizontally first};
\node [root,below of = p3] (p4) {\tiny switch(no. of bounding boxes)};
\node[proc1,below of = p4,xshift=-50mm,yshift=-35mm] (c1) {\tiny Single BBOX fills the entire image};
\node[proc1,below of = p4, xshift = -17mm,yshift=-35mm] (c2) {\tiny Place the 2 BBOX's horizontally by their side};
\node[proc1,below of = p4, xshift = 17mm,yshift=-35mm] (c3) {\tiny The BBOX with the largest height is placed in a separate column and the other two bounding boxes are placed vertically stacked horizontal to the first BBOX};
\node[proc1,below of = p4, xshift = 50mm,yshift=-35mm] (c4) {\tiny BBOX with the largest height and 3rd largest height are placed in the first column stacked vertically. BBOX's with 2nd largest and 4th largest height are placed in the second column stacked vertically.};
\path (p0.south) to node [near start, xshift=1em] {} (p1);
  \draw [->] (p0.south) -- (p1); 
\path (p1.east) to node [near start, xshift=0.3em, yshift=1em] {\tiny $No$} (p2);
  \draw [*->] (p1.east) -- (p2); 
\path (p1.south) to node [near start, xshift=1.2em] {\tiny $Yes$} (p3);
  \draw [*->] (p1.south) -- (p3);
\path (p3.south) to node [near start, xshift=1em] {} (p4);
  \draw [->] (p3.south) -- (p4);
\path (p4.south) to node [near start, xshift=0.3em] {\tiny $1$} (c1);
  \draw [->] (p4.south) -- (c1);
\path (p4.south) to node [near start, xshift=0.3em] {\tiny $2$} (c2);
  \draw [->] (p4.south) -- (c2);
\path (p4.south) to node [near start, xshift=0.3em] {\tiny $3$} (c3);
  \draw [->] (p4.south) -- (c3);
\path (p4.south) to node [near start, xshift=0.3em] {\tiny $4$} (c4);
  \draw [->] (p4.south) -- (c4);
\end{tikzpicture}
  \caption{Flowchart detailing the layout procedure. Please refer to figure \ref{fig:illustration} to observe the results of the layout procedure. The cases with 1,2 and 4 non-overlapping bounding boxes have been illustrated in figure \ref{fig:illustration}}
  \label{fig:tiling}
\end{figure*}
\section{Experimental Methodology}
\label{sec:experiment}
The ImageNet object detection dataset (DET) is a dataset comprising 200 classes of objects which is a subset of the ImageNet 1000 classes. Further, the ImageNet video object detection dataset (VID) comprises of 30 classes of objects which is a subset of the DET 200 classes. The ImageNet video object detection (VID) dataset was the most appropriate choice for illustrating the results of our work. The ImageNet VID training set has 3862 video snippets and the ImageNet VID validation set has 555 video snippets. 53539 frames from the DET dataset comprising only of the classes from the VID dataset and 57834 frames from the VID training set were combined to form the final training set. 
%This information is summarized in figure \ref{tab:dataset}. 
\par 
The SSD300 \cite{liu2016ssd} object detector operated on a per-frame basis was used as the baseline for our work. The SSD300 object detector uses VGG16 as feature extractor. The SSD300 pretrained model on the DET dataset was further trained on our training set for 210k iterations with a learning rate of $10^{-3}$ for the first $80000$ iterations, $10^{-4}$ for the next $40000$ iterations and $10^{-5}$ for the rest of the training. This SSD300 trained model gave a mAP score of $70.6$ on the VID validation set. Further, this model has a network throughput of $47$ fps and a overall throughput (including standard pre-processing time) of $18$ fps.
%\par
%\begin{figure}
%\begin{centering}
%\begin{tabular}{|p {2cm}|p {1cm} |p {1cm} |p {1cm} |}
%\hline 
%Dataset & No. of classes & No. of video snippets & No. of frames selected\tabularnewline
%\hline 
%\hline 
%DET training set & 200 & N/A & 53539\tabularnewline
%\hline 
%VID training set & 30 & 3862 & 57834\tabularnewline
%\hline 
%VID validation set & 30 & 555 & 176126\tabularnewline
%\hline 
%\end{tabular}\caption{Details of the ImageNet DET and ImageNet VID dataset}\label{tab:dataset}
%\par\end{centering}
%\end{figure}
One might suppose that we need two object detectors for our framework - one for higher sized images and one for lower sized images. The SSD300 network processes images at $300\times300$ as the name suggests. However, closer observation of the network suggested that the same network can process $150\times150$ images as well by stopping processing at the penultimate layer. Hence, we use the same SSD300 network with the same weights to process both higher sized images and lower sized images. In all our experiments, the baseline size $s_{1}$ is $300$ and the final lower size $s_{3}$ is $150$. When a $150\times150$ sized image is passed on to the SSD300 network, processing is configured to stop at the penultimate layer. All the experiments were performed using the SSD Caffe framework in a 2.1 GHz Intel Xeon CPU with a  Nvidia TITAN X GPU. Code will be released soon. In all the experiments, the batch size was $1$ to emulate an online setup. The detection threshold $\tau$ used to select ROIs was fixed at $0.2$ in most of our experiments unless explicitly specified otherwise.
\section{Experimental Results}
\label{sec:results}
\subsubsection*{Results from sample videos}
We show results on processing some sample videos with PaD. In figure \ref{fig:illustration}, we show some sample detections with our ROI-packing algorithm. The first column shows frame $i$. The second column shows the ROI packed frame $i+1$ with the detections. The third column shows the original frame $i+1$ with detections transformed from ROI packed frame $i+1$. For this experiment, the confidence threshold $\tau$ for selecting a detection as an ROI for the next frame is chosen as $0.3$ for the sake of illustration. All bounding boxes with a minimum threshold of $0.2$ are shown in the figure.
\begin{figure*}
\centering
%\advance\leftskip-3cm
%\advance\rightskip-3cm
\begin{tabular}{c|c|c}
Frame $i$ & ROI-packed frame $i+1$ & Frame $i+1$\\
\hline
\subfloat{\includegraphics[scale=0.15]{image1.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image2.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image3.JPEG}} \\[-0.3in]

\subfloat{\includegraphics[scale=0.15]{image4.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image5.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image6.JPEG}} \\[-0.3in]

\subfloat{\includegraphics[scale=0.15]{image7.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image8.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image9.JPEG}} \\[-0.3in]

\subfloat{\includegraphics[scale=0.15]{image10.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image11.JPEG}} &
\subfloat{\includegraphics[scale=0.15]{image12.JPEG}} \\

\end{tabular}
\caption{Sample set of consecutive frames processed with the ROI packing mechanism. The first column shows frame $i$. The second column shows the ROI packed frame $i+1$ with the detections. The third column shows the original frame $i+1$ with detections transformed from ROI packed frame $i+1$. For this experiment, the confidence threshold for selecting a detection as an ROI for the next frame is chosen as $0.3$ for the sake of illustration. All bounding boxes with a minimum threshold of $0.2$ are shown in the figure.}
\label{fig:illustration}
\end{figure*}
\par
In figures \ref{fig:tt}(a), we plot the time taken per frame for processing a sample video and the cumulative time taken for processing the same video using PaD and compare it with the baseline. It can be seen that processing the lower sized frame of $150\times150$ is almost $3\times$ faster. When ROI-packing fails, there is a slight overhead incurred which is visible towards the end of the video in figure \ref{fig:tt}(a). Also, we see that some frames require almost $0$s for processing. This is because the previous frame had no detections. Overall, we note that processing the video using PaD requires almost $8$s lesser time than the baseline from figure \ref{fig:tt}(b).
\begin{figure*}
  \centering
  \begin{tabular}{cc}
  \subfloat[]{\includegraphics[scale=0.4]{Videoprocess1_arrow.png}} &
\subfloat[]{\includegraphics[scale=0.35]{Videoprocess2.png}} \\
  \end{tabular}
  \caption{(a)Time taken per frame for processing a sample video (b)Cumulative time taken processing a sample video}
  \label{fig:tt}
\end{figure*}

\subsubsection*{Results over the entire dataset}
PaD was run with a inter-anchor distance $d=5$ and $s_{2}=150$. In figure \ref{fig:tpvpf}, we plot the histogram of average per-frame processing time on a video-by-video basis. In other words, the average time taken per frame was obtained for each video and is plotted as a histogram. From the figure, we can clearly see that the average time taken to process a frame is lower using PaD for more videos than the baseline. The baseline mAP score is $70.6$ and our method has a mAP score of $69.5$. Thus the mAP score drops by less than $1.6\%$ and $1.1$ percentage points. The average per-frame speedup is around $1.25 \times$. The average overhead incurred for ROI-packing is around $9\%$ of the total time taken.
\begin{figure}
  \centering
  \includegraphics[scale=0.4]{tpvpf_hist.png}
  \caption{Histogram of average per-frame processing time on a video-by-video basis}
  \label{fig:tpvpf}
\end{figure}
\subsubsection*{Comparison with a naive ROI-packing algorithm}
In order to illustrate the benefits of our sophisticated ROI-packing algorithm discussed in section \ref{sec:Methodology}, we compare the accuracy drop when compared with a naive ROI-packing algorithm.
\par
The naive ROI-packing algorithm works as follows. The naive ROI-packing algorithm can accommodate upto four ROI's just like the sophisticated method. If there are more than four objects in the frame, the frame is processed at full size. Otherwise, the bounding box surrounding each frame is extended by a factor of $1.2\times$ and is treated as an ROI. If there is only one object, the ROI surrounding the bounding box is rescaled to size $s_{3} \times s_{3}$ and is processed by the detector. If there are two objects, the lower sized frame is divided into two columns of size $s_{3} \times \frac{s_{3}}{2}$. The two ROIs are rescaled to the appropriate sizes and laid out on the lower sized frame. In the case of three or four objects, the lower sized frame is divided into four regions in two columns and two rows of size $\frac{s_{3}}{2} \times \frac{s_{3}}{2}$. In the case of three ROIs, the ROIs will be rescaled to occupy three of the four regions in the frame and the fourth region will be left blank. In the case four ROIs, the ROIs will be rescaled and fit to these four regions. We do not perform a greedy expansion of the RoIs to provide background context. Instead, the ROIs are just expanded by a constant factor of $1.2 \times$ and rescaled to appropriate size.
\par
Our sophisticated ROI packing method with inter-anchor distance $d=5$ gave a mAP score of $69.5$. With the same parameter setting, the naive ROI packing algorithm gave a mAP score of $56.8$. This clearly illustrates the need for a sophisticated ROI packing algorithm that preserves the scale and aspect ratio of the ROIs and provides as much background context as possible. Further, each object should be present in only one ROI to prevent redundant detections. This clearly shows that the CNN object detectors, though fairly robust to small scale changes cannot handle large variations in scale and are particularly sensitive to the aspect ratio. Also, CNN object detectors are overfit to the background context.
\subsubsection*{Tradeoff between speed and accuracy by parameter variation}
In figure \ref{fig:tradeoff1}, we vary the inter-anchor distance $d$  with $s_{2}=150$ and observe the effect on mAP score and speed. As $d$ is varied from $2$ to $10$, the mAP drops from $70.1$ to $68.9$ while the FLOP count reduction relative to the baseline increases from $18\%$ to $39\%$ on average over the entire validation set. Thus, the inter-anchor distance can be tuned according to the speed-accuracy tradeoff desired.
\begin{figure*}
  \centering
  \begin{tabular}{cc}
  \subfloat{\includegraphics[scale=0.3]{map_iad.png}} &
\subfloat{\includegraphics[scale=0.3]{speed_iad.png}} \\
  \end{tabular}
  \caption{Figure depicting the speed-accuracy tradeoff achieved by varying the inter-anchor distance}
  \label{fig:tradeoff1}
\end{figure*}
\par
The parameters $s_{1}=300$ and $s_{3}=150$ are decided by the specific CNN detector that is being used. However, the factor $s_{2}$ could be varied to obtain higher speeds. As $s_{2}$ is increased, the chances of the ROIs fitting in the lower sized layout increases, which in turn increases the chances of processing the frame at lower size. The speed-accuracy tradeoff with variation in $s_{2}$ is plotted in figure \ref{fig:tradeoff2}. With increase in $s_{2}$ from $150$ to $200$, the average FLOP count reduction relative to the baseline varies from $32\%$ to $44\%$. The average per-frame speedup increases from $1.21\times$ to $1.33\times$. However, there is relatively a high drop in accuracy to $6\%$ relative to the baseline at $s_{2}=200$. This shows that the CNN object detector though fairly robust to scale variations cannot handle large variations in scale.
\begin{figure*}
  \centering
  \begin{tabular}{cc}
  \subfloat{\includegraphics[scale=0.3]{map_scale.png}} &
\subfloat{\includegraphics[scale=0.3]{speed_scale.png}} \\
  \end{tabular}
  \caption{Figure depicting the speed-accuracy tradeoff achieved by varying the scaling factor}
  \label{fig:tradeoff2}
\end{figure*}
\section{Conclusion and Future Work}
\label{sec:conclusion}
Still-image object detection has improved by leaps and bounds in recent years due to the success in training and deploying neural networks. However, the opportunities that are available in the context of videos have not been fully exploited. Neural networks are in general very compute-hungry and inference can run in real-time in only the most high-end GPUs. In this work, we use the opportunities available in the context of videos to speed up and reduce the amount of computation in neural network object detectors. In PaD, the full-sized input will only be processed in anchor frames. In the inter-anchor frames, the ROIs in the frame are identified based on the location of the objects in the previous frame. These ROIs are packed together in a lower sized frame which is fed to the CNN object detector. The ROI packing algorithm needs to be sophisticated in the sense that it has to ensure that the scales and aspect ratios of the objects are preserved and enough background context is provided. With this setup, we observed $1.25 \times$ speedup with less than $1.6\%$ drop in accuracy on the ImageNet VID validation set. Further, the time taken to process a lower sized frame is almost $3 \times$ lesser and the FLOP count reduces by $4 \times$. Given more suitable datasets, we can get even more speedup and reduction in FLOP count in the average sense.
\par
As part of future work, we plan to incorporate a motion model to obtain the ROIs in the current frame. Incorporating a motion model could also help extend this framework to larger batch sizes. Also, it is possible to use two different models or networks to process larger sized and smaller sized frames. This will help reduce the accuracy drop but will in turn increase the memory footprint. There is an overhead incurred in checking whether the ROIs can fit in the lower sized frame. Currently, we select anchor frames at regular intervals. However, information on whether ROIs were packed successfully in previous frames can help us decide how frequently we select anchor frames. Thus, another line of future work is a dynamic mechanism for selecting anchor frames in order to reduce the overhead. Further, instead of using a heuristic hand-crafted algorithm for forming the ROI packed frame, a neural network could be trained to identify the ROIs and pack them in a lower sized frame like in an attention mechanism. This is another ambitious line of future work. It would be interesting to test PaD in more resource constrained platforms like mobile GPUs and CPUs. We expect the benefits to be more pronounced in such platforms.  

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigconf-xelatex.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-sigconf-xelatex.pdf:  sample-sigconf-xelatex.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	xelatex $<
	- bibtex $*
	xelatex $<
	xelatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do xelatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigconf-xelatex.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes
		
